ROME: Testing Image Captioning Systems via Recursive Object Melting

Image captioning (IC) systems aim to generate a text description of the salient objects in an image. In recent years, IC systems have been increasingly integrated into our daily lives, such as assistance for visually-impaired people and description generation in Microsoft Powerpoint. However, even the cutting-edge IC systems (e.g., Microsoft Azure Cognitive Services) and algorithms (e.g., OFA) could produce erroneous captions, leading to incorrect captioning of important objects, misunderstanding, and threats to personal safety. The existing testing approaches either fail to handle the complex form of IC system output (i.e., sentences in natural language) or generate unnatural images as test cases. To address these problems, we introduce Recursive Object MElting (Rome), a novel metamorphic testing approach for validating IC systems. Different from existing approaches that generate test cases by inserting objects, which easily make the generated images unnatural, Rome melts (i.e., remove and inpaint) objects. Rome assumes that the object set in the caption of an image includes the object set in the caption of a generated image after object melting. Given an image, Rome can recursively remove its objects to generate different pairs of images. We use Rome to test one widely-adopted image captioning API and four state-of-the-art (SOTA) algorithms. The results show that the test cases generated by Rome look much more natural than the SOTA IC testing approach and they achieve comparable naturalness to the original images. Meanwhile, by generating test pairs using 226 seed images, Rome reports a total of 9,121 erroneous issues with high precision (86.47%-92.17%). In addition, we further utilize the test cases generated by Rome to retrain the Oscar, which improves its performance across multiple evaluation metrics.

==> 00Abstract.tex <==
\begin{abstract}
Image captioning (IC) systems aim to generate a text description of the salient objects in an image.
In recent years, IC systems have been increasingly integrated into our daily lives, such as assistance for visually-impaired people and description generation in Microsoft Powerpoint.
However, even the cutting-edge IC systems (\textit{e.g.}, Microsoft Azure Cognitive Services) and algorithms (\textit{e.g.}, OFA) could produce erroneous captions, leading to incorrect captioning of important objects, misunderstanding, and threats to personal safety.
The existing testing approaches either fail to handle the complex form of IC system output (\textit{i.e.}, sentences in natural language) or generate unnatural images as test cases. 
To address these problems, we introduce \textit{Recursive Object MElting} ({\methodname}), a novel metamorphic testing approach for validating IC systems. 
Different from existing approaches that generate test cases by inserting objects, which easily make the generated images unnatural, {\methodname} \textit{melts} (\textit{i.e.}, remove and inpaint) objects.
{\methodname} assumes that the object set in the caption of an image includes the object set in the caption of a generated image after object melting.
Given an image, {\methodname} can recursively remove its objects to generate different pairs of images.
We use {\methodname} to test one widely-adopted image captioning API and four state-of-the-art (SOTA) algorithms.
The results show that the test cases generated by {\methodname} look much more natural than the SOTA IC testing approach and they achieve comparable naturalness to the original images.
Meanwhile, by generating test pairs using 226 seed images, {\methodname} reports a total of 9,121 erroneous issues with high precision (86.47\%-92.17\%).
In addition, we further utilize the test cases generated by {\methodname} to retrain the Oscar, which improves its performance across multiple evaluation metrics.


\end{abstract}



==> 01Introduction.tex <==
\section{Introduction}\label{sec:intro}



Image captioning (IC) systems, which generate a text description of the salient objects given an image, have been widely adopted in real-life scenarios.
For instance, the geographic information system (GIS) ArcGIS~\cite{arcgis_api} employs IC to describe the salient objects in remote sensing images for accessibility purposes.
Microsoft Edge Explorer uses IC to help visually-impaired individuals understand images on the web~\cite{edge_api}.
Meta Facebook utilizes IC to provide alternative texts for user photos~\cite{facebook_api}.  
These recent advances have been largely facilitated by the rapid development of deep neural networks in both computer vision (CV) and natural language processing (NLP)~\cite{vinyals_show_2015, xu_show_2015, li_oscar_2020, zhang_vinvl_2021, hu_vivo_2020, wang2022unifying}.
In particular, recent research~\cite{hu_vivo_2020} has claimed that the SOTA IC algorithm has achieved human-level performance in terms of CIDEr score~\cite{vedantam2015cider}.



\begin{figure}[ht]
		\centering
		\includegraphics[width=0.83\linewidth]{Figs/rome_recursive.pdf}
		\caption{The original image (1) and three images (2-4) generated by {\methodname} and the corresponding captions returned by VinVL~\cite{zhang_vinvl_2021}. Text in blue indicates the salient object(s) in the image, and text in red indicates caption error.}
		\label{fig:rome_recur_show}
		\vspace{-1em}
\end{figure}

Nevertheless, even top-notch IC systems are susceptible to generating incorrect captions, which can lead to severe misunderstandings, negative social consequences, or threats to personal safety~\cite{news_1_ai_nodate,ic2impariment,schroeder_microsoft_2016}.
Fig.~\ref{fig:rome_recur_show} presents four images and the corresponding captions generated by a recent IC algorithm~\cite{zhang_vinvl_2021}.
We can observe that the caption for image (4) "\textit{A window in a stone building with \underline{two} vases}") is incorrect since there is only one vase in the image.
According to media reports, the captions produced by current IC systems are often inaccurate or overly generic (\textit{e.g.}, incorrect gender or nationality)~\cite{ai_alttext_terrible}.
Additionally, a recent report by World Health Organization~\cite{organization_world_2019} shows that more than 2.2 billion people have vision impairment and they are expected to benefit from IC systems-powered AI assistants~\cite{ic2impariment,ic2impariment_2}.
However, since these IC systems can generate incorrect captions, AI assistants may return misleading messages, putting visually-impaired users at risk \cite{news_1_ai_nodate}.
Therefore, it is crucial to ensure the resilience and reliability of modern IC systems.

Developing an effective testing approach is a critical step towards achieving a robust image captioning (IC) system, similar to traditional software.
However, it is a challenging task due to several reasons.
Unlike traditional software, where the logic is predominantly expressed in the source code, the logic of IC systems is primarily encoded in the underlying neural network.
Consequently, code-based testing approaches~\cite{romdhana2021cosmo, viticchie2016assessment} designed for traditional software are not suitable for testing IC systems.
Furthermore, existing testing techniques for AI software mainly focus on software with a simple output format (\textit{e.g.}, a label for an image classifier).
In contrast, the output of an IC system is a natural language sentence, which is significantly more complex, rendering the ineffectiveness of existing approaches (\textit{e.g.}, metamorphic relations that assume the output label should be the same after perturbation).
The SOTA image captioning testing approach MetaIC~\cite{yu2022automated} achieved high precision in reporting suspicious issues.
In particular, MetaIC generates test cases by inserting an object into a specific position in a background image.
Due to the difficulty of finding a suitable insertion position, MetaIC often generates unnatural test cases (\textit{e.g.}, an image with "\textit{flying monkey around the moon}"), which are less likely to occur in the real world.



To tackle these challenges, we introduce \textit{recursive object melting} ({\methodname}), a novel, wide-applicable methodology for validating image captioning systems.
Different from the SOTA approaches that rely on object insertion to generate test cases, which can easily insert an object into an unsuitable position or with an unnatural size (\textit{e.g.}, a cat is larger than a plane), {\methodname} \textit{melt} an object.
Specifically, to melt an object, {\methodname} removes an object from an image and then conducts image inpainting (\textit{i.e.}, recover the missing part based on the remaining context of the image).
Our core idea is that the object set in the caption of an image should include the object set in the caption of a generated image after melting.
For example, in Fig.~\ref{fig:rome_recur_show}, the original image (\textit{i.e.}, image (1)) has four vases in a window.
When one vase was melted, we obtained the second image.
Intuitively, the objects in the caption of this generated image should be included in that of the original image.
However, we observed that object "balls" in the caption "\textit{A group of \underline{balls} sitting in a stone window}" was not included in the object set of the original image, indicating a potential error in either the caption of the original image or that of the generated image.
Based on this idea, {\methodname} recursively melts the object in an image (\textit{e.g.}, the other three images in Fig.~\ref{fig:rome_recur_show}) and constructs multiple image pairs.
Accordingly, we realize {\methodname} as two metamorphic relations (MRs): (1) \textit{object melt}: the object set of a melted image is the subset of that of the image before melting; (2) \textit{class melt}: an object class should not be in the caption if all the objects in that class were melted.
Specifically, {\methodname} automatically melts images by LaMa~\cite{suvorov2022resolution}, an advanced image inpainting technique, and identifies the object names from the captions by Stanza's POS Tagging technique~\cite{stanza}.
If the captions of the image pair returned by the IC system violate any of these MRs, the image pair and the corresponding captions will be reported as a suspicious issue.

To evaluate the effectiveness of {\methodname}, we use it to test one commercial API (\textit{i.e.}, Microsoft Azure Cognitive Services) and four SOTA IC algorithms (\textit{i.e.}, OFA~\cite{wang2022unifying}, Oscar~\cite{li_oscar_2020}, VinVL~\cite{zhang_vinvl_2021}, Attention~\cite{xu_show_2015}).
Based on a user study, test cases generated by {\methodname} are significantly more natural compared to those produced by the SOTA IC testing algorithm~\cite{yu2022automated}.
In the user study, annotators rated the naturalness of the test cases on a scale from 1 (unnatural) to 4 (natural), and the naturalness ratings were 3.33 \textit{vs.} 1.41 and 3.33 \textit{vs.} 1.37 for two running modes of the SOTA IC testing algorithm MetaIC~\cite{yu2022automated}.
{\methodname}'s test cases were even reported to be almost as natural as the original images (3.33 \textit{vs.} 3.56).
By generating test pairs from 226 seed images, {\methodname} reports 9,121 erroneous issues with high precision (86.47\%-92.17\%), which is comparable to the SOTA approach.
Meanwhile, we adopt {\methodname} to unveil labeling errors of COCO Caption~\cite{chen2015microsoft}, and successfully report 219 labeling errors.
In addition, we leverage the test cases generated by {\methodname} to retrain the Oscar base model, which improves its performance in terms of BLEU-4 (1.5\%), METEOR (3.4\%), CIDEr (2.0\%), and SPICE (7.9\%). The source code and the dataset of this paper will be publicly released.


This paper makes the following main contributions.
\begin{itemize}
    \item The introduction of a novel, widely-applicable methodology, recursive object melting ({\methodname}), for image captioning software validation;
    \item A practical implementation of {\methodname} by using LaMa~\cite{suvorov2022resolution} for image inpainting and leveraging Stanza's POS Tagging~\cite{stanza} for object name identification. 
    \item Empirical results demonstrating the effectiveness of {\methodname}: {\methodname} achieves comparable precision (86.47\% $\sim$92.17\%) to the SOTA approach~\cite{yu2022automated}, and the test cases generate by {\methodname} are much more natural (3.33 \textit{vs.} 1.26) in terms of human-annotated naturalness score.
\end{itemize}


==> 02Background.tex <==
\section{Preliminaries}\label{sec:bg}


\subsection{Image Captioning Algorithms}
Typically, IC is an image-to-sequence problem, where the input is image pixels and the output is natural language sentences. 
Previously, IC algorithms mainly entailed description retrieval~\cite{pan2004automatic, farhadi2010every,ordonez2011im2text} and hand-crafted natural language generation approaches~\cite{aker2010generating, li2011composing, yang2011corpus}.
With the development of deep learning, modern IC algorithms contain two steps: (1) \textit{visual encoding}: encode the input as one or multiple feature vectors; (2) \textit{sentence generation}: decode the intermediate representations into a sequence of words or sub-words according to a vocabulary. There are mainly two lines of IC systems: LSTM-based IC and multimodal pretraining IC. For LSTM-based IC, researchers proposed the single-layer LSTM~\cite{vinyals_show_2015}, two-layer LSTM~\cite{donahue2015long}, and LSTM with additive attention graph~\cite{xu_show_2015}.

In this paper, we mainly test multimodal pretraining IC algorithms, which have been developed rapidly in recent years~\cite{lu2019vilbert, chen2020uniter, gan2020large}.
Oscar~\cite{li_oscar_2020} adopts a BERT-like architecture that utilizes object tags as anchors to ease the semantic alignment between images and texts. 
Based on Oscar, VinVL~\cite{zhang_vinvl_2021} enhances feature extraction by adopting a specifically designed object detection component. OFA~\cite{wang2022unifying} achieves SOTA performance by unifying several vision and language tasks via a sequence-to-sequence learning framework, which has a unified instruction-based task representation.



\subsection{Motivating Examples}
\label{subsec:motivating_example}
Most of the SOTA testing approaches for IC and its related tasks generate test cases by inserting an object into a seed image. 
In particular, MetaOD~\cite{wang2020metamorphic}, which is the SOTA testing approach for object detection, inserts an object to a location that does not overlap with existing objects in the seed image. 
MetaIC~\cite{yu2022automated}, the SOTA testing approach for IC systems, inserts an object into a background image after location tuning and object resizing. 
Although these approaches perform well in finding erroneous outputs, the test cases generated by them are often unnatural.
For example, Fig.~\ref{fig:metaic_failure} demonstrates two test cases generated by MetaIC, where it inserts a horse into the image on the left and a spoon into the image on the right.
We can observe that even MetaIC provides location tuning and object resizing strategies, the images are still unnatural.
The left-hand side image inserts a horse into an inappropriate location (\textit{i.e.}, on the roof), while the right-hand side image inserts an oversized spoon, making it larger than a human.

In this paper, naturalness refers to how likely it is for an image to appear in the real world. While we think the unnatural test cases generated by MetaIC are still useful, we argue that IC systems are mainly used for natural images (\textit{e.g.}, assistance for visually-impaired people) and whether an IC system can provide correct captions for natural images is more important.
\begin{figure}[t]
		\centering
		\includegraphics[width=0.98\linewidth]{Figs/modify_metaicNonNat.pdf}
		\caption{A motivating example of test cases generated by MetaIC.}
		\label{fig:metaic_failure}
\end{figure}

